Social Media Emotions and Market Behavior

I explore the relationship between investor emotions expressed on social media and asset prices. The field has seen a proliferation of models aimed at extracting firm-level sentiment from social media data, though the behavior of these models often remains uncertain. Against this backdrop, my study employs EmTract, an open-source emotion model, to test whether the emotional responses identified on social media platforms align with expectations derived from controlled laboratory settings. This step is crucial in validating the reliability of digital platforms in reflecting genuine investor sentiment. My findings reveal that firm-specific investor emotions behave similarly to lab experiments and can forecast daily asset price movements. These impacts are larger when liquidity is lower or short interest is higher. My findings on the persistent influence of sadness on subsequent returns, along with the insignificance of the one-dimensional valence metric, underscores the importance of dissecting emotional states. This approach allows for a deeper and more accurate understanding of the intricate ways in which investor sentiments drive market movements.

==> Tables/trading_strategy_portfolio.tex <==
\begin{table}[htbp]\centering
\footnotesize
\begin{threeparttable}
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Trading Strategy \label{tab:trading_strategy}}
\begin{tabular}{l*{8}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}\\
                    &\multicolumn{1}{c}{Quintile 1}&\multicolumn{1}{c}{Quintile 2}&\multicolumn{1}{c}{Quintile 3}&\multicolumn{1}{c}{Quintile 4}&\multicolumn{4}{c}{Quintile 5}\\
\hline
&&&&&&&&\\[\dimexpr-\normalbaselineskip+2pt]
Mkt-RF              &     -0.0012         &      0.0330         &      0.0246         &     -0.0014         &      0.0251         &      0.0771         &     -0.0294         &      0.0090         \\
                    &    (0.0685)         &    (0.0592)         &    (0.0761)         &    (0.0574)         &    (0.0790)         &    (0.0831)         &    (0.1247)         &    (0.0606)         \\
&&&&&&&&\\[\dimexpr-\normalbaselineskip+2pt]
SMB                 &     -0.0536         &     -0.2339\sym{***}&     -0.0889         &      0.1939\sym{*}  &      0.0304         &     -0.0611         &      0.0449         &      0.0064         \\
                    &    (0.1045)         &    (0.0886)         &    (0.1267)         &    (0.1062)         &    (0.1254)         &    (0.1517)         &    (0.1916)         &    (0.0816)         \\
&&&&&&&&\\[\dimexpr-\normalbaselineskip+2pt]
HML                 &      0.1708\sym{*}  &      0.0331         &     -0.0525         &      0.0139         &     -0.2759\sym{**} &     -0.1095         &     -0.4496\sym{***}&     -0.0853         \\
                    &    (0.1015)         &    (0.0962)         &    (0.1370)         &    (0.1207)         &    (0.1125)         &    (0.1596)         &    (0.1695)         &    (0.0792)         \\
&&&&&&&&\\[\dimexpr-\normalbaselineskip+2pt]
MOM                 &      0.0127         &     -0.0222         &     -0.0469         &      0.0719         &     -0.0846         &      0.1963\sym{*}  &     -0.2609\sym{**} &      0.0073         \\
                    &    (0.0735)         &    (0.0702)         &    (0.0847)         &    (0.0816)         &    (0.0853)         &    (0.1099)         &    (0.1281)         &    (0.0600)         \\
&&&&&&&&\\[\dimexpr-\normalbaselineskip+2pt]
\alpha          &     -0.1212\sym{**} &      0.0339         &      0.1364\sym{**} &      0.1604\sym{***}&      0.2395\sym{***}&      0.0985         &      0.3843\sym{***}&      0.1982\sym{***}\\
                    &    (0.0551)         &    (0.0526)         &    (0.0587)         &    (0.0543)         &    (0.0588)         &    (0.0624)         &    (0.1025)         &    (0.0418)         \\
\hline
\hline
&&&&&&&&\\[\dimexpr-\normalbaselineskip+2pt]
Year $<$ 2016         &                     &                     &                     &                     &                     &           X         &                     &                     \\
Year $>=$ 2016        &                     &                     &                     &                     &                     &                     &           X         &                     \\
Winsorized          &                     &                     &                     &                     &                     &                     &                     &           X         \\
Observations        &   2842        &   2842        &   2842        &   2842        &   2842        &   1501        &   1341        &   2786        \\
$R^2$               &      0.0014         &      0.0022         &      0.0004         &      0.0018         &      0.0025         &      0.0048         &      0.0060         &      0.0009         \\
\hline\hline
\hline\hline
\end{tabular}
\begin{tablenotes}
\footnotesize 
\item Notes:  Robust standard errors in parentheses. \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\). Trading strategy sorts S\&P super-composite stocks with pre-market emotion data into quintiles based on level of aggregate happiness and fear for each calendar day. The zero-cost quintile j portfolio purchases stocks in the jth quintile of investor enthusiasm, and shorts equal amount of stocks in the jth quintile of investor fear (that are not already purchased). 
\end{tablenotes}
\end{threeparttable}
\end{table}



